MYTE: Morphology-Driven Byte Encoding for Better and Fairer Multilingual Language Modeling

A major consideration in multilingual language modeling is how to best represent languages with diverse vocabularies and scripts. Although contemporary text encoding methods cover most of the world's writing systems, they exhibit bias towards the high-resource languages of the Global West. As a result, texts of underrepresented languages tend to be segmented into long sequences of linguistically meaningless units. To address the disparities, we introduce a new paradigm that encodes the same information with segments of consistent size across diverse languages. Our encoding convention (MYTE) is based on morphemes, as their inventories are more balanced across languages than characters, which are used in previous methods. We show that MYTE produces shorter encodings for all 99 analyzed languages, with the most notable improvements for non-European languages and non-Latin scripts. This, in turn, improves multilingual LM performance and diminishes the perplexity gap throughout diverse languages.

==> figures/bpeb_delta.tex <==
\begin{figure}[!tb]
\centering
    \includegraphics[width=\linewidth]{figures/large_delta.png}
    \caption{The difference in Byte-per-English-Bit between \myt{} and \byt{} large models against compression factor of \ours{}. For each sentence, the BPEB value is normalized by the number of UTF-8 bytes used to represent the corresponding English sentence.
    Spearman's $\rho=-0.81$ Pearson's $\rho=-0.96$.
    }
    
    %normalized by the number of predicted UTF bytes across languages (standard Bits per Byte) for masked suffix prediction on mc4 dataset. Morphological encoding visibly outperforms the regular UTF one.
    \label{fig:bpeb-delta}
\end{figure}

==> figures/compression_rates.tex <==
\begin{figure*}[!tb]
    \centering
    \includegraphics[width=\textwidth]{figures/compression_mytes.png}
    \caption{Sequence compression rates on FLORES 200 from decomposition and subsequent morph merging \hg{use the name of the method instead} in comparison with the original utf-8 encoding.}
    \label{fig:comp-rates}
\end{figure*}

==> figures/lm_flores_scaling.tex <==
\begin{figure*}[!tb]
    \centering   \includegraphics[width=\textwidth]{figures/nlls_no_context_en_normed_scales.png}
    \caption{Snetence prediction superisal expressed as the normed NLL score on multi-parallel FLORES-200 corpus. The comparison shows that the large model demonstrates lower surprisals than the small myT5 model. The base model does not hold to the trend.}
    \label{fig:lm-flores-scaling}
\end{figure*}

==> tables/scrips.tex <==
\begin{table*}[!tb]
\small
\begin{tabular}{@{}llllll@{}}
\toprule
\multirow{2}{*}{Group ID} & \multirow{2}{*}{Group Name} & \multirow{2}{*}{Unicode Scripts}                                             & \multicolumn{3}{c}{Initial Byte for Codepoint}   \\ \cmidrule(l){4-6} 
                          &                             &                                                                              & 2 b            & 3 b            & 4 b            \\ \midrule
0                         & Latin                       & Latin                                                                        & \bytebox[]{42} & \bytebox[]{4A} & \bytebox[]{52} \\
1                         & Common                      & Mixed, Common, Inherited, Unkown                                             & \bytebox[]{43} & \bytebox[]{4B} & \bytebox[]{53} \\
2                         & Non-latin Alphabetic        & Greek, Cyrillic, Armenian, Georgian                                          & \bytebox[]{44} & \bytebox[]{4C} & \bytebox[]{54} \\
3                         & Abjads                      & Hebrew,  Arabic,  Syriac,  Thaana,  Tifinagh                                 & \bytebox[]{45} & \bytebox[]{4D} & \bytebox[]{55} \\
4                         & Abugidas North              & Devanagari, Gurmukhi, Gujarati, Oriya, Bengali, Sinhala, Tibetan             & \bytebox[]{46} & \bytebox[]{4E} & \bytebox[]{56} \\
5                         & Abugidas South              & Telugu, Kannada, Tamil, Malayalam, Thai,  Lao, Myanmar,  Tai, Tagalog, Khmer & \bytebox[]{47} & \bytebox[]{4F} & \bytebox[]{57} \\
6                         & CJK Logographs              & Hangul, Han, Yi, Katakana, Hiragana, Bopomofo                                & \bytebox[]{48} & \bytebox[]{50} & \bytebox[]{58} \\
7                         & Other                       & Remaining scripts                                                            & \bytebox[]{49} & \bytebox[]{51} & \bytebox[]{59} \\ \bottomrule
\end{tabular}
\label{results_per_language}
\end{table*}
